Neural-Symbolic Commonsense Reasoner with Relation Predictors

Commonsense reasoning aims to incorporate sets of commonsense facts, retrieved from Commonsense Knowledge Graphs (CKG), to draw conclusion about ordinary situations. The dynamic nature of commonsense knowledge postulates models capable of performing multi-hop reasoning over new situations. This feature also results in having large-scale sparse Knowledge Graphs, where such reasoning process is needed to predict relations between new events. However, existing approaches in this area are limited by considering CKGs as a limited set of facts, thus rendering them unfit for reasoning over new unseen situations and events. In this paper, we present a neural-symbolic reasoner, which is capable of reasoning over large-scale dynamic CKGs. The logic rules for reasoning over CKGs are learned during training by our model. In addition to providing interpretable explanation, the learned logic rules help to generalise prediction to newly introduced events. Experimental results on the task of link prediction on CKGs prove the effectiveness of our model by outperforming the state-of-the-art models.

==> backup_method.tex <==
%\subsection{Background Theory}
%\textit{Markov Blanket} of a variable $n \in N$, denoted as $MB(n)$, is a minimal set of variables conditioned on which all other variables are probabilistically independent of the target $n$ \citep{tsamardinos2003algorithms}. This property shields variable $n$ from the rest of variables $\{m | m \in N - \{n\} - MB(n)\}$, and limits it interaction to the neighbouring variables. This property means that considering the variables in $MB(n)$ is sufficient for knowing the probability of variable $n$. Hence, $MB(n)$ provides adequate information for optimal classification. 
%\subsection{Theoretical Framework}
Given a CKG $G$, probabilistic reasoning is concerned with finding a set of triples $\mathcal{T}$ that maximises the likelihood of the query $q$ with the distribution $Pr(q | G) = \sum_{\mathcal{T} \in \mathcal{G}} Pr(q | \mathcal{T}) Pr(\mathcal{T} | G)$, where $\mathcal{G}$ denotes a space of all ground clauses derived from $B$. $q$ can be expanded to $q = (y, t)$ where $y \in \{1, 0 \}$ is the label of a triple $t$, indicating whether $t$ is in $G$ or not. 
The corresponding optimisation problem becomes
\begin{equation}
    \label{eq:op_problem}
    \arg\max_{\mathcal{T} \in \mathcal{G}} Pr(y = 1 , t| \mathcal{T}) Pr(\mathcal{T} | G)
\end{equation}
In boolean logic, $Pr(G | B)$ is either 1 if the proof to the query is true, otherwise 0. In contrast, in the setting of probabilistic reasoning, there is a probability associated with the truth value of a ground clause. Thus, we consider the same solution as in Problog~\cite{} that there is a probability $Pr(y = 1 | c, G)$ of being true associated with each ground clause $c$, given ground clauses $G$. There is also a probability $Pr(c | G)$ of seeing a ground clause $c$ given a set of ground clauses $G$. For example, there are many follow-up events of \textit{eatIn(MARKUS, STARBUCKS)}, $Pr(c | G)$ denotes the probability of one of those events. Both terms give a meaningful explanation of $Pr(y = 1 , c| G) = Pr(y = 1| c, G) Pr(c|G)$ besides mathematical derivation. Then the optimisation problem \eqref{eq:op_problem} becomes
\begin{equation}
    \arg\max_{G \in \mathcal{G}} Pr(y = 1 |c, G) Pr(c| G, B) Pr( G | B)
\end{equation}

Weak unification operator allows to unify two clauses from the clause space $\mathcal{C}$ by comparing their representations using a similarity function $s : \mathcal{C} \times \mathcal{C} \rightarrow [0,1]$. Let $c$ be a ground clause, its probability of unification with respect to the background theory $B$ defined in~\cite{weber2019nlprolog} is:
\begin{equation}
    Pr( c | B) = \max_{c' \in B} s(c , c')
\end{equation}
where $s(c, c')$ is defined (w.r.t. the representation of each clause) as:
\begin{equation}
    s(c, c') = \frac{1}{2}\Big( 1 + \frac{\mathbf{v}_c^{\intercal}\mathbf{v}_{c'}}{\|\mathbf{v}_c\|\|\mathbf{v}_{c'}\|}\Big)
\end{equation}
If all atoms in the background theory is not always true, we extend them with their probabilities
\begin{equation}
    Pr(c | B) = \max_{c' \in B} s(c , c') Pr(y = 1| c', B)
\end{equation}
where $\mathbf{v}_c, \mathbf{v}_{c'}$ denote the representations of $c$ and $c'$, respectively, to have probabilistic version of weak unification.

Probabilistic weak unification can also be applied in the reasoning process. Taking backward chaining as an example, at step $t$, we have derived a ground clause set $G_{t-1}$ from the step $t-1$, for a given clause $c$, its probability of truthfulness is 
\begin{align*}
\label{eq:reason_weak_unify}
Pr(c| MB(G_{t-1}), B) = & \max_{c' \in MB(G_{t-1}) \cup B} s(c,c')\\ 
& Pr(y = 1| c', B)
\end{align*}. 
If there are $T$ steps to prove a query clause $c$, the joint probability of a proof chain $G$ is:
\begin{align*}
     Pr(c|MB(G), B) &  = Pr(q | MB(G_T))\\ 
     & \prod_{t=1}^T  Pr(MB(G_{t})| MB(G_{t-1}), B)
\end{align*}
Let $G_{t}/ MB(G_{t-1})$ denote a set of newly derived clauses from $MB(G_{t-1})$, we have
\begin{align*}
    & Pr(G_{t}| MB(G_{t-1}), B) = \\
    & \prod_{c \in G_{t}/ MB(G_{t-1})} Pr(c| MB(G_{t-1}), B)
\end{align*}
When we marginalize over all possible proof chains, we get
\begin{equation}
    Pr(c|B) = \sum_{G}Pr(q | G)\prod_{t=1}^T Pr(G_{t}| MB(G_{t-1}), B)
\end{equation}
We say $c$ is true when $Pr(q|B) > \lambda$, where $\lambda \in (0, 1]$ is a pre-specified threshold.


At the core of the reasoning process is the estimation of $Pr(y = 1|c, MB(G), B)$ and $Pr(c| MB(G_{t-1}), B)$.

The estimation of $Pr(c| MB(G_{t-1}), B)$ is based on probabilistic weak unification (see Eq. \eqref{eq:reason_weak_unify}).


The representation of events are provided by an sentence encoder $g(e)$, which is a deep language model such as BERT~\cite{devlin2018bert} fine tuned on background knowledge base. The details of fine tuning will be introduced in Sec.~\ref{sec:rep_learning}.

The background knowledge base is large, hence we can apply locality sensitive hashing~\cite{andoni2015lsh} or hierarchical navigable small world graphs~\cite{malkov2018nnHierarchical} to retrieve the neighbours of a ground clause.


Pre-trained deep neural networks, such as BERT~\cite{devlin2018bert}, take a pair of sentences as input, produce a continuous vector as their joint representation. Such models show promising performance of capturing associations between two input sentences. In this work, we apply BERT to encode each pair of sentences into a continuous vector $\mathbf{h}_{CLS}$ by using the representation of CLS. Then we pass $\mathbf{h}_{CLS}$ through an MLP as in~\cite{sap2019socialiqa} to get a joint representation $\mathbf{h}_j$.
\begin{equation}
\label{eq:hidden_joint_sens}
    \mathbf{h}_j = \mathbf{W}_2 \tanh(\mathbf{W}_1 \mathbf{h}_{CLS} + \mathbf{b})
\end{equation}
The probability $Pr(y = 1|c)$ for a particular predicate $p$ is computed by
\begin{equation}
\label{eq:prob_joint_sens}
    \sigma(\mathbf{w}_{p}^{\intercal} \mathbf{h}_j)
\end{equation}
where $\sigma(\cdot)$ is the sigmoid function.

To address the sparsity issue, we extend Atomic by first extracting new events, persona, and mental states from a large corpus, followed by classifying relations between them into the nine inference dimensions.



\subsubsection{Rules}
In this work, the rule sets for both evaluation corpora are small so that we manually compile the rules for them. The rule set for COPA consists of three rules:
\begin{align}\nonumber
    \text{causeOf}(A, B) \land \text{causeOf}(B, C) \implies \text{causeOf}(A,C)\\ \nonumber
    \text{causeOf}(A, B) \implies {resultOf}(B, A) \\ \nonumber
     \text{resultOf}(A, B) \land \text{resultOf}(B, C) \implies \text{resultOf}(A,C)\\   
\end{align}
The rule set for Atomic has up to three rules associated with each inference dimension:
\begin{align} \nonumber
    \text{xNeed}(A, B) \land \text{xNeed}(B, C) \implies \text{xNeed}(A,C)\\ \nonumber
     \text{xIntend}(A, B) \implies \text{xNeed}(A, B) \\ \nonumber
     \text{xNeed}(A, B) \implies \text{xWant}(B, A) \\ \nonumber
    ... 
\end{align}

In the future, we can apply inductive logic programming (ILP) to find rules to deal with applications requiring complex rule sets. Given a background theory $B$, ILP is concerned with finding a set of definite clauses $H$ from a set of positive and negative examples $P$ and $N$. Probabilistic ILP is then to find the set of definite clauses $H$ that maximizes the likelihood of the data $Pr(E | H, B)$, where $E = P \cup N$.
\begin{equation}
    \label{eq:ilp}
    Pr(E | H , B) = \prod_{(y,e) \in E} Pr((y, e) | H , B)
\end{equation}
where $y \in \{0 , 1\}$ is the label of an example $e$. In commonsense causal reasoning on events, we consider the following rule templates:
\begin{align}\nonumber
    Q(A,B) &\implies P(B,A)\\
    Q(A,B) &\implies P(A,B)\\
    Q(A,B) \land R(B,C) &\implies P(A, C)
\end{align}
where $P, Q, R$ are replaced by the predicates in the background knowledge base.

Given a hypothesis space $\mathcal{H}$, probabilistic ILP with weak unification is formulated as the following optimization problem.
\begin{equation}
    \arg\max_{H \in \mathcal{H}} Pr(E | H, B) Pr(H | B)
\end{equation}
